Large-Signal Stability Guarantees for Cycle-by-Cycle Controlled DC-DC Converters

Stability guarantees are critical for cycle-by-cycle controlled dc-dc converters in consumer electronics and energy storage systems. Traditional stability analysis on cycle-by-cycle dc-dc converters is incomplete because the inductor current ramps are considered fixed; but instead, inductor ramps are not fixed because they are dependent on the output voltage in large-signal transients. We demonstrate a new large-signal stability theory that treats cycle-by-cycle controlled dc-dc converters as a particular type of feedback interconnection system. An analytical and practical stability criterion is provided based on this system. The criterion indicates that the L/R and RC time constants are the design parameters that determine the amount of coupling between the current ramp and the output voltage.

==> test.tex <==
\section{Modeling of Boost Converter}
\subsection{Overall System}
Consider a class $\Sigma$ boost converter defined in \cite{Cui2018a}, which uses the constant on-time current-mode control as illustrated in Fig.\,\ref{fig:cotcm_buck}. The output voltage is sampled during the on-time, once per switching cycle. The sampling time point for $v[n]$ can be expressed as the convex combination of the time of the inductor current valley $t_v[n]$ and the time for the inductor current peak $t_p[n]$
\begin{figure}
    \centering
    \includegraphics[width = 7cm]{cotcm_buck.pdf}
    \caption{Constant on-time buck converter using cycle-by-cycle current-mode control.}
    \label{fig:cotcm_buck}
\end{figure}
\begin{align}
t_s[n] = \lambda t_v[n-1] + (1-\lambda)t_p[n],
\end{align}
the parameter $\lambda$ can be chosen to be from 0 to 1.

The slopes of the rising and falling ramps of inductor current are denoted by $m_1[n]$ and $m_2[n]$
\begin{subequations}
\begin{align} 
    m_1[n] &= \frac{V_{\text{in}}}{L},  \label{eqn:m1n}  \\
    m_2[n] &= \frac{v[n]-V_{\text{in}}}{L}. \label{eqn:m2n} 
\end{align}
\end{subequations}

We introduce the one-cycle-delayed peak current sequence $\{i_p^p[n]\}$ as
\begin{align}
    i_p^p[n+1] &\triangleq i_p[n]. \label{eqn:ivp}
\end{align}

We denote the equilibrium of system by $v[n] = V_{\text{out}}$, $i_v[n] = I_{v}$, $i_p^p[n] = I_{v}$, and $t_\text{off}[n] = T_{\text{off}}$. The equilibrium is defined by the following equations:
\begin{subequations}
\begin{align}
    I_v & = \frac{V_{\text{out}}}{R} - \frac{1}{2}\frac{V_{\text{in}}-V_{\text{out}}}{L}T_{\text{on}}, \label{eqn: equlibrium1} \\
    T_{\text{off}} & = \frac{V_{\text{in}}-V_{\text{out}}}{V_{\text{out}}} T_{\text{on}}, \,\,\, T_{s}^{\text{ss}} = T_{\text{off}} + T_{\text{off}} , \label{eqn: equlibrium2}\\
    I_v & = I_c - w(T_{\text{off}}). \label{eqn: equlibrium3}
\end{align}
\end{subequations}


\subsection{Current Block Modeling}
The large-signal dynamical model of the current block is
\begin{subequations}
\begin{align}
    i_p^{p}[n+1] & = i_p^{p}[n] + m_1[n]t_{\text{on}} - m_2[n]T_{\text{off}}, \label{eqn:toff} \\
    i_p^{p}[n+1]  & = i_c[n] - w(t_{\text{on}}[n]).
\end{align}
\end{subequations}
The equilibrium is translated to the origin 
%substitute (\ref{eqn:qin1}), (\ref{eqn:qin2}), (\ref{eqn:qout}), \ref{eqn:toff}, and (\ref{eqn: equlibrium1}) into (\ref{eqn:v_dyn}), 
\begin{subequations} \label{eqn:i_tilde_dyn}
\begin{align}
    \tilde{i}_p^{p}[n+1] & = \tilde{i}_p^{p}[n] - \frac{\tilde{v}[n]}{L}T_{\text{off}} + \frac{V_{\text{in}}}{L}\tilde{t}_{\text{on}}[n], \\
    \tilde{i}_p^{p}[n+1]  & = \tilde{i}_c[n] - \psi(\tilde{t}_{\text{off}}[n]),
\end{align}
\end{subequations}
where 
%$t_{\text{off}}[n]$ is the off time described by (\ref{eqn:toff}),
$\tilde{v}[n]$, $\tilde{i}_p^p[n]$, $\tilde{t}_{\text{off}}[n]$, and $\psi$ satisfy
\begin{subequations}
    \begin{align}
        \tilde{v}[n] &= v[n] - V_{\text{out}}, \label{eqn:v_dev}\\
        \tilde{i}_p^p[n] &= i_p^p[n] - I_v, \label{eqn:i_dev} \\
        \tilde{t}_{\text{off}}[n] &= t_{\text{off}}[n] - T_{\text{off}}, \label{eqn:toff_dev} \\
        \psi(x) &= w(x+T_{\text{off}}[n]) - w(x). \label{eqn:psi} 
    \end{align}
\end{subequations}
From (\ref{eqn:i_tilde_dyn}), the current block diagram can be outlined as Fig.\,\ref{fig:Current_block}.
\begin{figure}[ht]
    \centering
    \includegraphics[width=7cm]{Current_block.pdf}
    \caption{Current block diagram.}
    \label{fig:Current_block}
\end{figure}
\subsection{Voltage Block Modeling}
%We made two reasonable assumptions for power electronics to simplify the %derivation: 
Class $\Sigma$ buck converter has the following two properties:
(1) the output RC-filter time constant is much greater than the switching period; (2) the output voltage has a small ripple so the inductor current can be considered as cycle-varying piecewise linear (ramp) waveform. The property (1) contains
\begin{align} \label{eqn:assumption_1}
    \frac{T_s[n]}{RC} \ll 1,
\end{align}
where $T_s$ is the switching period at the $n^{\text{th}}$ switching cycle. The property (2) contains the {\em{quasi-steady state discharging}}, i.e. the discharging current to the load can be treated as constant every switching cycle, and {\em{small output-voltage ripple}} 
\begin{align} \label{eqn:assumption_2}
    \frac{T_{s}[n]T_{\text{on}}}{2LC} & \ll 1.  
\end{align}

The large-signal dynamical model of voltage block follows \cite{Cui2018a}: 
\begin{subequations}
\begin{align}
    v[n+1] &= v[n] + \frac{1}{C}\left(\sum_{j=1}^3Q^{(j)}_{\text{in}}[n] - Q_{\text{out}}[n]\right), \label{eqn:v_dyn} \\
    Q^{(1)}_{\text{in}}[n] &= \left( i_p^p[n] + \frac{1 + \lambda }{2} m_1[n] T_{\text{on}}\right) (1-\lambda) T_{\text{on}}, \label{eqn:qin1}\\
    Q^{(2)}_{\text{in}}[n] &= \frac{1}{2}\left( i_p^p[n] + m_1[n]T_{\text{on}} +  i_p^p[n+1] \right)t_{\text{off}}[n], \label{eqn:qin2} \\
    Q^{(3)}_{\text{in}}[n] &= \left( i_p^p[n+1] + \frac{\lambda }{2}  m_1[n] T_{\text{on}} \right) \lambda T_{\text{on}}, \label{eqn:qin3}\\
    Q_{\text{out}}[n] &= \frac{v[n]}{R}\left( T_{\text{on}} + t_{\text{off}}[n]\right) \label{eqn:qout}.
\end{align}
\end{subequations}
The equilibrium is translated to the origin 
%We translate the states to the origin, 
%substitute (\ref{eqn:qin1}), (\ref{eqn:qin2}), (\ref{eqn:qout}), \ref{eqn:toff}, and (\ref{eqn: equlibrium1}) into (\ref{eqn:v_dyn}), 
%the dynamical model of the voltage block then follows
\begin{subequations} \label{eqn:tilde_dyn}
\begin{align}
    \tilde{v}[n+1] = \,\,& \tilde{v}[n] + \frac{1}{C}\left(\sum_{j=1}^3\tilde{Q}^{(j)}_{\text{in}}[n] - \tilde{Q}_{\text{out}}[n]\right), \label{eqn:tildev_dyn} \\
    \tilde{Q}^{(1)}_{\text{in}}[n] = \,\,& (1-\lambda) T_{\text{on}} \tilde{i}_p^p[n] - \frac{1 - \lambda^2}{2} \frac{\tilde{v}[n]}{L} T^2_{\text{on}}, \label{eqn:tildeqin1}\\
    \tilde{Q}^{(2)}_{\text{in}}[n] = \,\,& \frac{1}{2}\left( \tilde{i}_p^p[n] -\frac{\tilde{v}[n]}{L}T_{\text{on}} +  \tilde{i}_p^p[n+1] \right)t_{\text{off}}[n] \nonumber \\
    &+ \left(I_v + \frac{M_1T_{\text{on}}}{2}\right)\tilde{t}_{\text{off}}[n], \label{eqn:tildeqin2} \\
    \tilde{Q}^{(3)}_{\text{in}}[n] = \,\,& \lambda T_{\text{on}}  i_p^p[n+1] - \frac{\lambda^2}{2}  \frac{\tilde{v}[n]}{L} T^2_{\text{on}},  \label{eqn:tildeqin3}\\
    \tilde{Q}_{\text{out}}[n] = \,\,& \frac{\tilde{v}[n]}{R}\left( T_{\text{on}} + t_{\text{off}}[n] \right) +\frac{V_{\text{out}}}{R} \tilde{t}_{\text{off}}[n]. \label{eqn:tildeqout}
\end{align}
\end{subequations}
% where $t_{\text{off}}[n]$ is the off time described by (\ref{eqn:toff}), $\tilde{v}[n]$, $\tilde{i}_p^p[n]$, and $\tilde{t}_{\text{off}}[n]$ satisfy
% \begin{subequations}
%     \begin{align}
%         \tilde{v}[n] &= v[n] - V_{\text{out}} \label{eqn:v_dev}\\
%         \tilde{i}_p^p[n] &= i_p^p[n] - I_v \label{eqn:i_dev} \\
%         \tilde{t}_{\text{off}}[n] &= t_{\text{off}}[n] - T_{\text{off}} \label{eqn:toff_dev} 
%     \end{align}
% \end{subequations}
To avoid the switching transient disturbing the valley current detection, the time varying off-time is bounded from below. To avoid the misdetection on the valley current event, the time varying off-time is bounded from above as
\begin{align} \label{eqn:toff_bd}
    T^{\text{min}}_{\text{off}} \le t_{\text{off}}[n] \le T^{\text{max}}_{\text{off}}.
\end{align}
\section{Stability and Control Performance Analysis}
\subsection{Current Block}
To calculate the $\mathcal{L}_2$ gain from $\tilde{v}[n]$ to $\tilde{i}_p^p[n]$, denoted by $\Gamma_{v \to i}$, we introduce the following dissipativity theory.
\begin{figure}
    \centering
    \includegraphics[width = 3.5cm]{Lft_general.pdf}
    \caption{Linear fractional transformed system.}
    \label{fig:Lft_general}
\end{figure}
If the system can be converted in $F_u(L,\Delta)$ form \cite{Jonsson1996}, as shown in Fig.\,\ref{fig:Lft_general}, and
% \begin{figure}
%     \centering
%     \includegraphics[width = 5 cm]{Figure/section2/General_lft.png}
%     \caption{Linear fractional transformed system.}
%     \label{fig:General_lft}
% \end{figure}
the state-space representation of $F_u(L,\Delta)$ is
\begin{subequations}
    \begin{align}
        x[n+1] & = A x[n] + B_1 h[n] + B_2 r[n], \\
        p[n] & = C_1 x[n] + D_{11} h[n] + D_{12} r[n], \\
        e[n] & =  C_2 x[n] + D_{21} h[n] + D_{22} r[n], \\
        h[n] & = \Delta \, \left( p[n] \right),
    \end{align}
\end{subequations}
the upper bound of the $\mathcal{L}_2$ gain can be calculated as
\begin{theorem} \label{theorem:lure_gain}
Assume $\Delta$ is a $[\hat{\alpha}, \hat{\beta}]$ sector-bounded nonlinearity. Also, assume $F_u(L,\Delta)$ is well-posed. If $\exists \, P > 0$, $\lambda \ge 0$ and $\hat{\gamma} > 0$ such that
\begin{align}
    & \begin{bmatrix}
        A^TPA - P &   A^TPB_1 &   A^TPB_2 \\
        B_1^TPA                & B_1^TPB_1 &   B_1^TPB_2 \\
        B_2^TPA                & B_2^TPB_1 &   B_2^TPB_2 - \hat{\gamma}^2 I
    \end{bmatrix} \nonumber \\
    & + \lambda \begin{bmatrix}
    C_1 & D_{11} & D_{12}\\
    0   & I      & 0  
    \end{bmatrix}^T 
    \begin{bmatrix}
    -\hat{\alpha} \hat{\beta} &  \frac{\hat{\alpha} + \hat{\beta}}{2} \\ 
    \frac{\hat{\alpha} + \hat{\beta}}{2} & -1
    \end{bmatrix} 
    \begin{bmatrix}
    C_1 & D_{11} & D_{12}  \\
    0   & I      & 0
    \end{bmatrix} \nonumber \\
    & + \begin{bmatrix}
    C_2^T \\
    D_{21}^T \\
    D_{22}^T 
    \end{bmatrix} 
    \begin{bmatrix}
    C_2 & D_{12} & D_{22}
    \end{bmatrix}
    <0,
\end{align}
then 
% (a) For any $x[n] = x_0$, the state $x[n] \rightarrow 0$ as $n \rightarrow 0$\\
$\|F_u(L,\Delta)\| \le \hat{\gamma}$.
\end{theorem}
\begin{proof}
Define the storage function $V(x)\triangleq x^T P x$. Multiply on the left/right by $\left[x[n]^T\,\,p[n]^T\,\,h[n]^T\right]$ and its transpose to obtain
\begin{align} \label{eqn:dissipation_ineqn}
V(x[n+1]) - V(x[n]) & + \lambda \left(h[n] - \hat{\alpha} p[n]\right)\left(\hat{\beta} p[n] - h[n]\right) \nonumber \\
& + \left( \hat{\gamma}^2 e[n]^2 - r[n]^2 \right) < 0.
\end{align}
The second term with $\hat{\alpha}$ and $\hat{\beta}$ is non-negative because the sector bounded nonlinearity and positive scalar term $\lambda$. By summing up both sides of the (\ref{eqn:dissipation_ineqn}), we have $\|e\|_2^2 < \hat{\gamma}^2 \|d\|_2^2 + V(x[1])$, hence the $\mathcal{L}_2$ norm of $F_u(L,\Delta)$ is bounded by $\hat{\gamma}$.
%By letting $r[n] = 0$, the third term with $\hat{\gamma}^2$ is non-negative. Thus implies $V(x[n+1]) - V(x[n]) < 0$.
\end{proof}
We reformulate the current block in a unitless $F_u(L, \Delta)$ form as
\begin{subequations} \label{eqn:unitless_current-block}
\begin{align}
    \tilde{i}_p^{p}[n+1] &= \tilde{i}_i[n], \\
    \tilde{i}_e[n] &= \tilde{i}_p^{p}[n] - \tilde{i}_i[n] + \tilde{u}[n], \\
    \tilde{i}_p^{p}[n] &= \tilde{i}_p^{p}[n],\\
     \tilde{i}_i^{p}[n] &= \Delta (\tilde{i}_e[n]),
\end{align}
\end{subequations}
where
\begin{align}
     \tilde{u}[n] &= \frac{T^{\text{ss}}_{s}}{L} \tilde{v}[n],\\
     \Delta(z) &= -\psi \left(\frac{z}{m_2[n]} \right), 
\end{align}
and $\Delta(z) \in [\hat{\alpha}, \hat{\beta}]$ is a sector bounded time-varying nonlinearity. 

From Theorem \ref{theorem:lure_gain}, the gain $\hat{\gamma}$ of unitless $F_u(L, \Delta)$ form can be estimated by the following optimization problem:
\begin{subequations} \label{optproblem:currentgain}
\begin{align}
\underset{\hat{\gamma}, \lambda, P}{\mathrm{min}}& \,\,\,  \hat{\gamma}^2  \\
\text{subject to} & \,\, P>0, \,  \lambda\ge 0,\,  \hat{\gamma} >0 \label{eqn:opt_layer1_contraint1},\\
    &  \lambda \begin{bmatrix}
        - \hat{\alpha}\hat{\beta} & \hat{\alpha}\hat{\beta} + \frac{\hat{\alpha}+\hat{\beta}}{2}  &  -\hat{\alpha}\hat{\beta} \\
        \hat{\alpha}\hat{\beta} + \frac{\hat{\alpha}+\hat{\beta}}{2}   & - 2\hat{\alpha}\hat{\beta} -\hat{\alpha}-\hat{\beta} & \hat{\alpha}\hat{\beta} + \frac{\hat{\alpha}+\hat{\beta}}{2}    \\
        -\hat{\alpha}\hat{\beta}   & \hat{\alpha}\hat{\beta} + \frac{\hat{\alpha}+\hat{\beta}}{2} &  -\hat{\alpha}\hat{\beta}
    \end{bmatrix} \nonumber \\
    & + \begin{bmatrix}
        1 - P &  0 &  0 \\
        0  & P &   0 \\
        0   & 0 &  - \hat{\gamma}^2
    \end{bmatrix} < 0. \label{eqn:opt_layer1_contraint2}
\end{align}
\end{subequations}
Problem (\ref{optproblem:currentgain}) is in linear matrix inequality (LMI) form, hence is convex and the global minimum exists. By applying a LMI solver (e.g. CVX), we obtain the gain of system (\ref{eqn:unitless_current-block}) as a function of sector bounds,
\begin{align}  
    \hat{\gamma} = g(\hat{\alpha}, \hat{\beta}).
\end{align}
If no interference, $\hat{\alpha} = \hat{\beta} = 0$, system (\ref{eqn:unitless_current-block}) has zero gain, and voltage doesn't affect the current. As $\hat{\alpha}$ decreases and $\hat{\beta}$ increases, the system (\ref{eqn:unitless_current-block}) has larger gain, as shown in Fig.\,\ref{fig:Current_block_gain}.

\begin{figure}
    \centering
    \includegraphics[scale = 1]{Current_block_gain.png}
    \caption{Gain of system (\ref{eqn:unitless_current-block}) as a function of sector bounds. If no interference, $\hat{\alpha} = \hat{\beta} = 0$, system (\ref{eqn:unitless_current-block}) has zero gain, and voltage doesn't affect the current. As $\hat{\alpha}$ decreases and $\hat{\beta}$ decreases, the system (\ref{eqn:unitless_current-block}) has larger gain.}
    \label{fig:Current_block_gain}
\end{figure}
As a conclusion, the $\mathcal{L}_2$ of the current block is bounded from above by 
\begin{align}\label{egn:gamma_vi}
    \Gamma_{v \to i} \le \frac{T_s^{\text{ss}}}{L} g(\hat{\alpha}, \hat{\beta}),
\end{align}
where $T_s^{\text{ss}}$ is the steady-state switching period.
% \begin{align}
%     T_s^{\text{ss}} &\triangleq T_{\text{on}} +  T_{\text{off}}^{\text{ss}}.
% \end{align}
\subsection{Voltage Block}
\subsubsection{Voltage Block Model Reformulation}
The voltage dynamics, which is described by the nonlinear time-invariant system (\ref{eqn:tilde_dyn}), is a nonlinear system with quadratic and fractional nonlinearity. There does not exist a straightforward mathematical tool to analytically study the stability and calculate the $\mathcal{L}_2$ gain. The algorithmic method only applies to a specific buck converter with specific $L$, $C$, and $R$. Therefore, it is hard to generalize the algorithmic methods and give engineering intuitions to the designers.

We solve this challenge by taking use of the inherent physical constraint in the constant on-time power converter that the cycle-varying off-time is bounded as (\ref{eqn:toff_bd}).
\begin{theorem}
Given the class $\Sigma$ buck converter modeled by \cite{Cui2018a}, the $\mathcal{L}_2$ gain from the one-cycle-delayed inductor current sequence $\{\tilde{i}^{p}_v[n]\}$ to sampled output voltage sequence $\{\tilde{v}[n]\}$ is bounded from above as
\begin{align}
    \Gamma_{i \to v} &  \le \frac{R}{\left( 1 + \frac{T_{\text{on}}}{2\tau_2}\right)} \frac{T_s^{\text{max}}}{T_s^{\text{min}}},
\end{align}
where $T_s^{\text{min}}$ and $T_s^{\text{max}}$ are the shortest switching period and longest switching period, respectively, and $\tau_2$ is the $L-R$ time constant,
\begin{align}
    T_s^{\text{max}} & \triangleq T_{\text{on}} +  T_{\text{off}}^{\text{max}}, \\
    T_s^{\text{min}} & \triangleq T_{\text{on}} +  T_{\text{off}}^{\text{min}},\\
    \tau_2 &\triangleq \frac{L}{R}.
\end{align}
\end{theorem}

\begin{proof}
The nonlinear time-invariant system (\ref{eqn:tilde_dyn}) can be converted to the following linear time-varying system
\begin{subequations}
\begin{align}
       \tilde{v}[n+1] &= \alpha[n]\,\tilde{v}[n] +  \beta[n]\,\tilde{i}_p^p[n] + \gamma[n]\,\tilde{i}_p^p[n+1] ,\\
       \alpha[n] &= 1-\frac{T_{\text{on}}+t_{\text{off}}[n]}{RC}-\frac{T_{\text{on}}\left( T_{\text{on}} + t_{\text{off}}[n] \right)}{2LC},\\
       \beta[n] &= \frac{1}{C} \left( (1-\lambda ) T_{\text{on}} + \frac{1}{2} t_{\text{off}}[n] \right), \\
       \gamma[n] &= \frac{1}{C} \left( \lambda T_{\text{on}} + \frac{1}{2} t_{\text{off}}[n] \right).
    \end{align}
\end{subequations}
From (\ref{eqn:toff_bd}), the time-varying coefficient are bounded as
\begin{subequations}
\begin{align}
     0 < \alpha[n] & \le \alpha_{\text{max}} = 1 - \frac{T_{s}^{\text{min}}}{RC} - \frac{T_{\text{on}} T_{s}^{\text{min}}}{2LC},\\
     0 < \beta[n] & \le \beta_{\text{max}} = \frac{1}{C} \left( (1-\lambda) T_{\text{on}} + \frac{1}{2} T_{\text{off}}^{\text{max}} \right), \\
     0 < \gamma[n] & \le \gamma_{\text{max}} = \frac{1}{C} \left( \lambda T_{\text{on}} + \frac{1}{2} T_{\text{off}}^{\text{max}}  \right).
    % T_{s}^{\text{min}} & = T_{\text{on}} + T_{\text{off}}^{\text{min}}
\end{align}
\end{subequations}

We convert the linear time-varying system into the standard state-space representation
\begin{subequations}
\begin{align}
    \tilde{v}[n+1] &= \alpha[n]q[n] + \left( \beta[n]+ \alpha[n] \gamma[n] \right) \tilde{i}_p^p[n], \label{eqn:ivq2q} \\ 
    \tilde{v}[n] &=  q[n] + \gamma[n] \tilde{i}_p^p[n].  \label{eqn:ivq2v}
\end{align}
\end{subequations}
\subsubsection{Gain Estimation}
We utilize a storage function $\mathcal{V}[n] = q^2[n]$ to calculate the $\mathcal{L}_2$ gain of the dynamical system (\ref{eqn:ivq2q})
\begin{align} \label{eqn:storage_func_diff}
   \mathcal{V}[n+1]- \mathcal{V}[n] = q^2[n+1] - q^2[n].
\end{align}
From Cauchy-Schwartz Inequality, given any $\mu_1 > 0$, $ q^2[n+1]$ can be bounded from the above by
\begin{align}
 & q^2[n+1] \nonumber\\
=& \,\, \left( \alpha[n] q[n] + \left(\beta[n] + \alpha[n] \gamma[n]\right) \tilde{i}_p^p[n] \right)^2 \nonumber\\
\le& \,\,  \left( \alpha^2 [n] q^2[n] + (\beta[n] + \alpha[n] \gamma[n])^2
\frac{(\tilde{i}_p^p[n])^2}{\mu_1}\right) \left(1+\mu_1\right).
\end{align}
We let $\mu_1 = \alpha[n](1 - \alpha[n])^{-1}$. It can be verified that $\mu_1 > 0$ from (\ref{eqn:assumption_1}) and (\ref{eqn:assumption_2})
\begin{align} \label{eqn:qn_bd}
  & q^2[n+1] \le \alpha[n] q^2[n] + \frac{\left(\beta[n] + \alpha[n] \gamma[n]\right)}{1- \alpha[n]} (\tilde{i}_p^p[n])^2.
\end{align}
Substitute (\ref{eqn:qn_bd}) to (\ref{eqn:storage_func_diff}),
\begin{align}
    & \mathcal{V}[n+1]- \mathcal{V}[n] \nonumber \\
\le & \frac{\left(\beta[n] + \alpha[n] \gamma[n]\right)^2}{1- \alpha[n]} (\tilde{i}_p^p[n])^2 - (1 - \alpha[n]) q^2[n] \nonumber\\
\le & \frac{\left|\beta[n] + \alpha[n] \gamma[n]\right|_{\text{max}}^2}{1- \alpha[n]} (\tilde{i}_p^p[n])^2 - (1 - \alpha[n]) q^2[n] \nonumber\\
\le & \frac{\left(\beta_{\text{max}} + \alpha_{\text{max}} \gamma_{\text{max}}\right)^2}{1- \alpha_{\text{max}}} (\tilde{i}_p^p[n])^2 - (1 - \alpha_{\text{max}}) q^2[n] \nonumber \\
= & (1 - \alpha_{\text{max}}) \left( \frac{\left(\beta_{\text{max}} + \alpha_{\text{max}} \gamma_{\text{max}}\right)^2}{(1- \alpha_{\text{max}})^2} (\tilde{i}_p^p[n])^2 -  q^2[n] \right).
\end{align}
Sum both sides of the inequality for all $n$ yields
\begin{align}
    \mathcal{V}(\infty)- \mathcal{V}(1) \le (1 - \alpha_{\text{max}})\left(\Gamma_1^2 \|\tilde{i}_p^p\|_2^2 - \|q\|_2^2 \right),
\end{align}
where $\|\cdot\|$ is $\mathcal{L}_2$ norm and 
\begin{align}
    \Gamma_1 = \frac{\left(\beta_{\text{max}} + \alpha_{\text{max}} \gamma_{\text{max}}\right)}{(1- \alpha_{\text{max}})}. \label{eqn:gamma_1_def}
\end{align}
The $\mathcal{L}_2$ norm of $q[n]$ can be bounded by
\begin{align}
    \|q\|^2 & \le \Gamma_1^2  \|\tilde{i}_p^p\|_2^2 + \frac{V(1)-V(\infty)}{(1-\alpha_{\text{max}})} \nonumber \\
    & \le  \Gamma_1^2 \|\tilde{i}_p^p\|_2^2 + \frac{V(1)}{(1-\alpha_{\text{max}})}. \label{eqn:gain_q_gamma_1}
\end{align}
By definition, the $\mathcal{L}_2$ gain of system ($\ref{eqn:ivq2q}$) is bounded from above by $\Gamma_1$.

The $\mathcal{L}_2$ gain of the system (\ref{eqn:ivq2v}) can be estimated by Cauchy-Schwartz Inequality as 
\begin{align}
     & \tilde{v}^2[n] = (q[n] + \gamma[n] \tilde{i}_p^p[n])^2 \nonumber \\
     \le & \left( q^2[n] + \gamma^2[n] (\tilde{i}_p^p[n])^2 \frac{\Gamma_1}{\gamma[n]}\right)\left(1+\frac{\gamma[n]}{\Gamma_1}\right) \nonumber \\
     \le & \left(\Gamma_1 + \gamma[n]\right) \Gamma_1(\tilde{i}_p^p[n])^2 +   \left(\Gamma_1 + \gamma[n]\right) \gamma[n](\tilde{i}_p^p[n])^2 \nonumber\\
     \le & \left(  \Gamma_1 + \gamma_{\text{max}} \right) (\tilde{i}_p^p[n])^2.
\end{align}
% \begin{align}
%     \Gamma_{i \to v} = \Gamma_1 + \gamma_{\text{max}}. \label{eqn:gamma_2_def}
% \end{align}
Summing both sides of the inequality for all $n$ yields the $\mathcal{L}_2$ gain of the system (\ref{eqn:ivq2v})
\begin{align}
    \|v\|_2 \le \left(  \Gamma_1 + \gamma_{\text{max}} \right) \|\tilde{i}_p^p\|_2. \label{eqn:gain_i_v}
\end{align}
By (\ref{eqn:gamma_1_def}), the $\mathcal{L}_2$ gain of the voltage block can be bounded from above 
\begin{align} \label{egn:gamma_iv}
    \Gamma_{i \to v} & \le \Gamma_1 + \gamma_{\text{max}} = \frac{\beta_{\text{max}}+\gamma_{\text{max}}}{1-\alpha_{\text{max}}} =  \frac{R}{\left( 1 + \frac{T_{\text{on}}}{2\tau_2}\right)} \frac{T_s^{\text{max}}}{T_s^{\text{min}}},
\end{align}
where $T_s^{\text{min}}$ and $T_s^{\text{max}}$ are the shortest switching period and longest switching period, respectively, and $\tau_2$ is the $L-R$ time constant.
% \begin{subequations}
% \begin{align}
%     T_s^{\text{max}} &\triangleq T_{\text{on}} +  T_{\text{off}}^{\text{max}} \\
%     T_s^{\text{min}}& \triangleq T_{\text{on}} +  T_{\text{off}}^{\text{min}} \\
%     \tau_2 &\triangleq \frac{L}{R}
% \end{align}
% \end{subequations}
\end{proof}

\subsection{Overall System}
From Small Gain Theorem \cite{Okuyama2014}, the current-mode buck converter is finite-gain $\mathcal{L}_2$ stable if
\begin{align} \label{eqn:sgt_sys}
    \Gamma_{i\to v} \cdot \Gamma_{v\to i} < 1.
\end{align}
By substituting (\ref{egn:gamma_vi}) and (\ref{egn:gamma_iv}) into (\ref{eqn:sgt_sys}), $\ref{eqn:sgt_sys}$ is equivalent to
\begin{align}
    g(\hat{\alpha}, \hat{\beta}) < \left(\tau_2 + \frac{T_{\text{on}}}{2}\right)\frac{T_s^{\text{min}}}{T_s^{\text{max}}} \frac{1}{T_s^{ss}},
\end{align}
where $T_s^{\text{min}}$, $T_s^{\text{max}}$, and $T_s^{\text{ss}}$ are the shortest switching period, longest switching period, and steady-state switching period, respectively.

Because both current and voltage blocks are zero state observable \cite{khalil2002nonlinear}, the finite-gain $\mathcal{L}_2$ stability implies the current-mode buck converter is large-signal asymptotically stable. 

\red{the result for current-mode buck converter using constant off time, current-mode boost converter using constant on time and }

